Illuminating the Physics of Cosmic Origin and Evolution: A UK Space Frontiers 2035 White Paper

Understanding the Universe's origins and evolution remains one of the most fundamental challenges in modern cosmology. This white paper explores three key science priorities in this field: unravelling the physics of cosmic inflation, investigating the accelerating expansion of the Universe, and precisely measuring the sum of the neutrino masses. Achieving these goals requires a dedicated survey to map the large-scale structure at high redshift in unprecedented detail. We describe how this can be achieved through a mission concept called SIRMOS, providing a high-throughput, highly multiplexed spectroscopic capability to obtain accurate redshifts for over 100 million galaxies over a wide sky area. Such a survey would leverage the deepest existing wide-area photometric catalogues for targeting, with spectra offering continuous 1.25-2.5~$\mu$m wavelength coverage at moderate resolution, allowing precise redshift measurements in the $1<z<4$ range with minimal bias. We outline the scientific opportunities this presents. Recent years have seen significant advances in instrumentation, including digital micromirror devices, complex telescope mirrors, large detector arrays, and data processing pipelines. While these technologies have been demonstrated in terrestrial applications, such a survey is a unique opportunity to apply these proven capabilities in space to address fundamental questions in cosmology. Participation in such a mission will simultaneously deliver a compelling science case, help align UK Space Agency and STFC strategies, demonstrate the UK's growing capability in end-to-end space missions, and strengthen the national space economy through high-value industrial participation.

==> abstract.tex <==
--------------------------------------
Version 1
--------------------------------------
SIRMOS is an Explorer mission concept that aims to illuminate the Physics of Cosmic Origins and Evolution. Its primary science goals are: (1) Discover how cosmic inflation seeded large-scale structure in the Universe. (2) Unveil the physics of cosmic acceleration. (3) Measure the sum of neutrino masses. SIRMOS focuses on two major science questions: What set the Hot Big Bang in motion? What physics drives the cosmic expansion and large-scale evolution of the Universe? In its 3-year prime mission, SIRMOS will execute a cosmology survey over the Euclid footprint of 14,000 sq deg, to obtain slit spectra for 100M galaxies at 1 < z < 4. To accomplish its transformative science goals, SIRMOS utilizes digital micro-mirror devices for spectroscopic target selection, achieving a multiplex of 4000 and spectral resolution R > 1000 from 1.25 to 2.5 microns. SIRMOS surveys will leverage Euclid photometry for target selection. We welcome community input and participation in SIRMOS science

--------------------------------------
Version 2
--------------------------------------
SIRMOS will revolutionize our understanding of the universe by mapping the large-scale structure of galaxies in unprecedented breadth and detail to explore cosmic origins and evolution. This NASA Explorer mission offers a unique opportunity for UK scientists to lead groundbreaking research in cosmology and for UK industry to contribute cutting-edge instrumentation in high-tech fields such as optics and detectors –- including complex telescope mirrors, advanced detector applications, data processing pipelines, or autonomous target acquisition. SIRMOS aims to discover how cosmic inflation seeded large-scale structure, reveal the nature of the accelerating expansion of the universe, and measure the sum of neutrino masses to exceptionally high precision.

In its 3-year prime mission, SIRMOS will execute a cosmology survey over the \textit{Euclid} footprint of $\sim$14,000~deg$^2$, obtaining slit spectra for 100,000,000 galaxies at $1<z<4$. SIRMOS is the first space mission designed specifically to leverage \textit{Euclid}'s wide near-IR imaging survey for target selection and the first to exploit digital micro-mirror devices to acquire 4,000 simultaneous spectra over a wide $1~\mathrm{deg}^2$ field of view. The instrument's excellent spectral resolution of $R>1000$ and continuous wavelength coverage from 1.25--2.5~$\mu$m captures the redshifts of distant galaxies with no gaps in coverage, minimizing systematic biases to achieve ground-breaking science. SIRMOS represents a compelling opportunity to advance UK leadership in space science and technology, offering significant benefits to both UK scientists and industry. \blue{EM: We need to walk a fine line here. "While the primary emphasis is on science priorities, papers may also address enabling missions, instrumentation, or technology development needed to realise the proposed goals. However, this is not a formal call for mission proposals or facilities. " To me this abstract reads too much of mission proposal rather than science white paper.
